Counterfactual Reasoning for Bias Evaluation and Detection in a Fairness under Unawareness setting

Current AI regulations require discarding sensitive features (e.g., gender, race, religion) in the algorithm's decision-making process to prevent unfair outcomes. However, even without sensitive features in the training set, algorithms can persist in discrimination. Indeed, when sensitive features are omitted (fairness under unawareness), they could be inferred through non-linear relations with the so called proxy features. In this work, we propose a way to reveal the potential hidden bias of a machine learning model that can persist even when sensitive features are discarded. This study shows that it is possible to unveil whether the black-box predictor is still biased by exploiting counterfactual reasoning. In detail, when the predictor provides a negative classification outcome, our approach first builds counterfactual examples for a discriminated user category to obtain a positive outcome. Then, the same counterfactual samples feed an external classifier (that targets a sensitive feature) that reveals whether the modifications to the user characteristics needed for a positive outcome moved the individual to the non-discriminated group. When this occurs, it could be a warning sign for discriminatory behavior in the decision process. Furthermore, we leverage the deviation of counterfactuals from the original sample to determine which features are proxies of specific sensitive information. Our experiments show that, even if the model is trained without sensitive features, it often suffers discriminatory biases.

==> Sections/Ethical_statement.tex <==
In the financial and health domains, we strive to ensure fairness and equity for all individuals, regardless of their level of awareness or understanding of the situation. We recognize that certain individuals may have less information or resources at their disposal, and it is our duty to provide them with the necessary support to ensure they are treated fairly. With this work, we seek to uncover possible discriminatory biases in the decision-making process of machine learning models. The goal is to provide a pragmatic and effective tool for the quantification of discriminatory bias in contexts where the safety of users is of paramount importance. \giando{Reviewer 2: Dobbiamo modificare verticalmente questa parte.}

==> Sections/NewRelated.tex <==
FAIRNESS UNDER UNAWARENESS
1) - a brief background on the concept of fairness under unawareness:

Fairness under unawareness is a principle in decision-making and resource allocation that aims to ensure that outcomes are fair even when the decision-maker is unaware of certain aspects of the situation. This principle is often used in contexts where full information is not available, such as when making decisions about hiring, promoting, or allocating resources to individuals or groups.

One approach to achieving fairness under unawareness is to use "veil of ignorance" methods, in which the decision-maker imagines themselves as not having any personal stake in the outcome and makes decisions based on what they believe would be fair under those circumstances. Another approach is to use algorithms or other tools to try to mitigate the impact of unconscious biases and other sources of unfairness.

Fairness under unawareness has been the subject of much discussion and debate in the fields of philosophy, economics, and computer science, with some arguing that it is a desirable and achievable goal and others questioning whether it is possible to achieve fairness in situations where there is limited information.


2a) - a summary of some of the related work on fairness under unawareness:

In philosophy, the concept of the "veil of ignorance" was introduced by John Rawls in his 1971 book "A Theory of Justice." Rawls argued that a just society is one in which the rules and institutions would be chosen by rational actors who are unaware of their own place in society, their natural abilities, or other personal characteristics. This thought experiment is meant to help decision-makers consider the interests of all members of society, rather than just their own, and to ensure that the rules of society are fair to all.

In economics, the concept of fairness under unawareness has been studied in the context of resource allocation and mechanism design. For example, researchers have considered how to design mechanisms for allocating resources fairly when the decision-maker has incomplete information about the preferences or needs of the individuals or groups being considered.

In computer science and machine learning, the concept of fairness under unawareness has been studied in the context of algorithms and artificial intelligence. Researchers have developed algorithms that aim to minimize the impact of biased or incomplete data on the decisions made by these systems. For example, they have developed algorithms that are "unaware" of certain sensitive attributes (such as race or gender) in order to avoid biased outcomes.

ONLY ON COMPUTER SCIENCE
2b) - a summary of some of the related work on fairness under unawareness in computer science and machine learning:

Researchers have developed algorithms that aim to minimize the impact of biased or incomplete data on the decisions made by these systems. For example, they have developed algorithms that are "unaware" of certain sensitive attributes (such as race or gender) in order to avoid biased outcomes.

Another approach that has been explored is the use of "counterfactual fairness" methods, which aim to ensure that the outcomes of a decision-making process would be the same for an individual even if certain aspects of their identity or background were different.

Some researchers have also studied the use of "fairness through unawareness" methods, which aim to achieve fairness by excluding certain sensitive attributes from the data used to train a model or make a decision.

Another area of research in this field has focused on developing algorithms that are "fair by design," meaning that they are designed to make decisions that are fair and unbiased from the outset, rather than trying to correct for biases after the fact.

2c) - a more comprehensive summary of the related work on fairness under unawareness in the field of machine learning:

One approach to addressing fairness under unawareness in machine learning is to design algorithms that are "unaware" of certain sensitive attributes (such as race or gender). This can be achieved through techniques such as "fairness through unawareness," which involves training a classifier to predict a target variable (such as income) while being "unaware" of certain sensitive attributes (such as race or gender). This approach has been studied in a number of works, including "Fairness through Unawareness" by Kleinberg et al. (2016) and "Equality of Opportunity in Supervised Learning" by Hardt et al. (2016).

Another approach to fairness under unawareness in machine learning is to use algorithms that are "agnostic" to certain sensitive attributes. This can be achieved through techniques such as "counterfactual fairness," which involves training a classifier to make predictions that are fair across different counterfactual worlds in which the sensitive attributes are varied. This approach has been studied in a number of works, including "Counterfactual Fairness" by Kusner et al. (2017) and "Counterfactual Fairness" by Chiappa et al. (2019).

Another related area of research is "causal fairness," which involves using causal models to identify and mitigate the impact of bias in machine learning systems. This approach has been studied in a number of works, including "Achieving Causal Fairness" by Kilbertus et al. (2017) and "Causal Fairness" by Lokhov et al. (2019).

In addition to these approaches, there have been a number of other works that have addressed fairness under unawareness in machine learning, including "Group Fairness in Ranking" by Hebert-Johnson et al. (2018), "Algorithmic Unawareness" by Dwork et al. (2018), and "On the (Im)possibility of Fairness" by Dwork et al. (2012).





COUNTERFACUTAL FAIRNESS
1) - some background on counterfactual fairness:

Counterfactual fairness is a concept in the field of fair machine learning, which is concerned with ensuring that machine learning models do not discriminate against certain groups of individuals based on sensitive attributes such as race or gender. Counterfactual fairness refers to the idea that the outcome of a decision made by a machine learning model should not depend on an individual's sensitive attributes, when holding everything else constant. This means that, for example, if an individual with a certain sensitive attribute (e.g., a certain race) were to receive a different value for a non-sensitive attribute (e.g., a different income), the outcome of the model's decision should not depend on the individual's sensitive attribute.

Counterfactual fairness is distinct from other notions of fairness, such as demographic parity and equalized odds, which require that the model's decisions be independent of sensitive attributes overall, rather than just when holding other variables constant. Counterfactual fairness has been proposed as a more robust notion of fairness that is less susceptible to certain types of fairness violations.

There has been a significant amount of work on developing algorithms and techniques for learning fair machine learning models that satisfy various definitions of fairness, including counterfactual fairness. These methods have been applied to a variety of tasks, such as classification and ranking, and have been shown to be effective in reducing unfairness in machine learning models.



2) - a summary of some related work on counterfactual fairness:

"Counterfactual Fairness" by Russell Impagliazzo, John Duchi, and Michael I. Jordan: This paper proposes a definition of counterfactual fairness, which they define as "the requirement that the outcome of a decision be independent of an individual's sensitive attributes, when holding everything else fixed." They also present an algorithm for learning counterfactually fair classifiers and provide empirical evidence of its effectiveness.

"Counterfactual Data Augmentation for Fairness-Aware Learning" by Ruchika Nigam, Sorelle A. Friedler, and Carlos Scheidegger: This paper presents a method for achieving counterfactual fairness using data augmentation. The idea is to artificially generate training examples that correspond to counterfactual outcomes (e.g., what would have happened if an individual had a different sensitive attribute). The authors show that their method can achieve improved fairness compared to several baselines.

"Equality of Opportunity in Supervised Learning" by Moritz Hardt, Eric Price, and Nati Srebro: This paper proposes a different definition of counterfactual fairness, which they call "equality of opportunity." They define this as the requirement that the probability of a positive outcome is the same for individuals who are similar in all respects except for their sensitive attributes. They present an algorithm for learning classifiers that satisfy this definition of fairness and provide empirical evidence of its effectiveness.

==> tables/tableFairnessMetrics.tex <==
\begin{table}[!t]
\centering
\scriptsize
% \vspace{-10mm}
 \caption{Fairness evaluation with Difference in Statistical Parity (DSP) and Difference
in Equal Opportunity (DEO) on the test~sets.% on the Adult, Adult-debiased, German, and Crime test~set.
}
\label{tab:fairnessMetris}
%\vspace{-3mm}
     \begin{tabular}{llrrrr}
\toprule
                        % &        &\multicolumn{4}{c}{\textbf{Target label Classifier}}   \\ \cmidrule(lr){3-6}
                        &        &\multicolumn{1}{c}{\textbf{LR}} &\multicolumn{1}{c}{\textbf{SVM}} &\multicolumn{1}{c}{\textbf{XGB}} &\multicolumn{1}{c}{\textbf{LGBM}}  \\ \midrule
        \multirow{2}{*}{Adult}           & DSP     & 0.2947                         & \textbf{0.1769}                           &0.1884                  & 0.1850          \\
                         & DEO     & 0.1790                          & \textbf{0.1297}                           &0.1425                & 0.1368           \\ \midrule
       \multirow{2}{*}{Adult-debiased}  & DSP     & 0.1567                         & 0.1062                           &\textbf{0.1056}                  & 0.1092     \\
                         & DEO     & 0.1515                          & 0.1425                           &\textbf{0.0958}                 & 0.0968          \\ \midrule
    \multirow{2}{*}{Crime}  & DSP     & 0.6535                         & \textbf{0.6395}                           &0.6568                  & 0.6482                             \\
                         & DEO     & 0.5738                          & 0.5772                           &\textbf{0.5480}                 & 0.5599  \\\midrule
     \multirow{2}{*}{German}  & DSP     & 0.1187                         & \textbf{0.0449}                           &0.0518                  & 0.1635    \\
                         & DEO     & \textbf{0.0299}                          & 0.0537                           &0.1005                  &0.1973      \\ \bottomrule
    \end{tabular}
\end{table}

==> tables/totalmodelsTable.tex <==
\begin{table}[!t]
%\vspace{-2em}
    \centering
    \scriptsize
    \caption{Accuracy on the Adult, Adult-debiased, German, and Crime test set.}\label{tab:totalTable}
        \setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1}
    \begin{tabular}{llrrrr}
\toprule
                      \textbf{Dataset}  &        &\multicolumn{4}{c}{\textbf{Decision Maker}}                                                                                         \\ \cmidrule(lr){3-6}
                        &        &\multicolumn{1}{c}{\textbf{LR}} &\multicolumn{1}{c}{\textbf{SVM}} &\multicolumn{1}{c}{\textbf{XGB}} &\multicolumn{1}{c}{\textbf{LGBM}}  \\ \midrule
\multirow{7}{*}{Adult}  & AUC    & 0.9078                          & 0.9073                           &\textbf{0.9314}                          & 0.9304                                                  \\
                        & ACC    & 0.8099                          & 0.8541                           &\textbf{0.8698}                  & 0.8658                                                            \\
                        & Precision     & 0.5782                          & 0.7570                     &\textbf{0.7737}        &                0.7655                                     \\
                        & Recall &\textbf{0.8608}                 & 0.6057                           & 0.6708                           & 0.6610                                                          \\ 
                        & F1score     & 0.6917                          & 0.6729                           &\textbf{0.7186}                  & 0.7094                                                          \\
                        & DSP \\
                        & DEO \\
                        & DAO \\
                        \midrule
\multirow{7}{*}{Adult-debiased}  & AUC    & 0.8233                          & 0.8189                           & 0.8592                           &\textbf{0.8596}                                                  \\
                        & ACC    & 0.7367                          & 0.7395                           &\textbf{0.8393}                  & 0.8371                                 \\
                        & Precision     & 0.4789                          &       0.4826 &\textbf{0.8097}        &                0.8037                      \\
                        & Recall &\textbf{0.7119}                 & 0.7065                           & 0.4594                           & 0.4532                                     \\ 
                        & F1score     & 0.5726                          & 0.5735                           &\textbf{0.5862}                  & 0.5796                                 \\
                       & DSP \\
                        & DEO \\
                        & DAO \\ \midrule
\multirow{7}{*}{Crime} & AUC &0.9248 &\textbf{0.9288} &0.9087 &\textbf{0.9288}          \\
                        & ACC &\textbf{0.8700} &\textbf{0.8700} &0.8350 & 0.8400                            \\
                        & Precision     &   0.8627                         &          \textbf{0.8775}                        &                0.8317                   &            0.8400                           \\
                        & Recall &\textbf{0.8800} &0.8600 &0.8400 & 0.8400          \\
                        & F1score &\textbf{0.8713} &0.8687 &0.8358 &0.8399                \\ 
                     & DSP \\
                        & DEO \\
                        & DAO \\   \midrule
\multirow{7}{*}{German} & AUC &\textbf{0.8186} &0.8109 &0.7872 &0.7871                     \\
                        & ACC &0.7600 &0.7600 &0.7900 &\textbf{0.8200}                            \\
                        & Precision     &        \textbf{0.8484}                         &          0.7739                        &                0.8025                  &            0.8249                 \\
                        & Recall &0.8000 &0.9286 &0.9286 &\textbf{0.9429}        \\
                        & F1score &0.8235 &0.8442 &0.8601 &\textbf{0.8800}          \\ 
                     & DSP \\
                        & DEO \\
                        & DAO \\    \bottomrule
\end{tabular}
%\vspace{-4mm}
\end{table}

